L1-aware Multilingual Mispronunciation Detection Framework

The phonological discrepancies between a speaker's native (L1) and the non-native language (L2) serves as a major factor for mispronunciation. This paper introduces a novel multilingual MDD architecture, L1-MultiMDD, enriched with L1-aware speech representation. An end-to-end speech encoder is trained on the input signal and its corresponding reference phoneme sequence. First, an attention mechanism is deployed to align the input audio with the reference phoneme sequence. Afterwards, the L1-L2-speech embedding are extracted from an auxiliary model, pretrained in a multi-task setup identifying L1 and L2 language, and are infused with the primary network. Finally, the L1-MultiMDD is then optimized for a unified multilingual phoneme recognition task using connectionist temporal classification (CTC) loss for the target languages: English, Arabic, and Mandarin. Our experiments demonstrate the effectiveness of the proposed L1-MultiMDD framework on both seen -- L2-ARTIC, LATIC, and AraVoiceL2v2; and unseen -- EpaDB and Speechocean762 datasets. The consistent gains in PER, and false rejection rate (FRR) across all target languages confirm our approach's robustness, efficacy, and generalizability.

==> tmp.tex <==
The phonological discrepancies between a speaker's native language (L1) and the target language (L2) serves as a major factor for mispronunciation. Traditionally designing mispronunciation detecting and diagnosis (MDD) often focus solely on L2-data for a single target language, hence neglecting the valuable insights that could be captured from multilingual target language modeling and L1-aware features. 

Therefore, this paper introduces a novel multilingual MDD (multi-MMD) architecture enriched with L1-aware speech representation. 
Using the L1-dependent multilingual latent space, the model learns to capture the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.
The multi-MMD model trained 



Utilizing an end-to-end transformer-based speech encoder architecture, the model is optimized in an end-to-end manner utilizing 
a unified multilingual phoneme output space. This is further augmented by embedding both L1 and L2 speech characteristics, which are solely extracted from the raw input speech, thereby offering a holistic approach to pronunciation assessment.

% become more sensitive to the idiosyncrasies of each language.
% capturing the nuanced influences of the speaker's linguistic background, thereby offering a more robust and comprehensive approach to pronunciation error detection in low-resource setting.

% that primarily supports English, Arabic, and Mandarin as target languages. This framework is enriched with L1-aware speech representation, capturing the nuanced influences of the speaker's linguistic background, thereby offering a more robust and comprehensive approach to pronunciation error detection in low-resource setting.


We demonstrates the generalizability using unseen datasets EpaDB, Speechocean762.


Our experiments shows that L1-dependent multilingual latent space able to capture 


the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


The multi-MDD is then optimized jointly for a unified phoneme output space for the following target languages --  English, Arabic, and Mandarin.

These results in a L1-dependent multilingual latent space and the model learns to capture the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


% We trained an end-to-end transformer-based speech encoder with an unified multilingual phoneme output space. further enriched with L1- and L2-speech embedding extracted from the raw input speech only. 


% his is further augmented by embedding both L1 and L2 speech characteristics, which are solely extracted from the raw input speech, thereby offering a holistic approach to pronunciation assessment.




An unified phoneme set is designed to train a transformer-based speech encoder that is further enriched with L1- and L2-speech embedding trained in an end-to-end manner. 


The framework is optimised 

phonetic representation is designed to train The multi-MMD model trained 



% Mispronunciation often result from contrasting phonological patterns between a speaker's native language (L1) and the target language (L2). 
The phonological discrepancies between the speaker's native language (L1) and the target language (L2) is one of the primary factors in mispronunciation. These contrasting patterns are often missing when modeling mispronunciation detection model using the available L2-data for a single target language overlooking the potential in multilingual target language modeling and L1-aware representations. This paper proposes a novel multilingual MDD architecture -- supporting mainly English, Arabic, and Mandarin, as target language.
% enhanced with L1-aware speech representation to characterize the intricacies of each target language phonology influenced by speakers' own nativity. 
% Our method enriches this paradigm by 
The proposed multilingual framework is enhanced with L1-aware speech representation, encapsulating the influence of speaker's own nativity.  

phonological patterns to enhance the robustness and accuracy of mispronunciation detection in multiple languages.
% along with lack of L2-data for the target language.
The paper proposes a novel multilingual MDD architecture that







% .  We demonstrates the generalizability using unseen datasets EpaDB, Speechocean762.


% Our experiments shows that L1-dependent multilingual latent space able to capture 


% the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


% The multi-MDD is then optimized jointly for a unified phoneme output space for the following target languages --  English, Arabic, and Mandarin.

% These results in a L1-dependent multilingual latent space and the model learns to capture the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


% % We trained an end-to-end transformer-based speech encoder with an unified multilingual phoneme output space. further enriched with L1- and L2-speech embedding extracted from the raw input speech only. 


% % his is further augmented by embedding both L1 and L2 speech characteristics, which are solely extracted from the raw input speech, thereby offering a holistic approach to pronunciation assessment.




% An unified phoneme set is designed to train a transformer-based speech encoder that is further enriched with L1- and L2-speech embedding trained in an end-to-end manner. 


% The framework is optimised 

% phonetic representation is designed to train The multi-MMD model trained 



% % Mispronunciation often result from contrasting phonological patterns between a speaker's native language (L1) and the target language (L2). 
% The phonological discrepancies between the speaker's native language (L1) and the target language (L2) is one of the primary factors in mispronunciation. These contrasting patterns are often missing when modeling mispronunciation detection model using the available L2-data for a single target language overlooking the potential in multilingual target language modeling and L1-aware representations. This paper proposes a novel multilingual MDD architecture -- supporting mainly English, Arabic, and Mandarin, as target language.
% % enhanced with L1-aware speech representation to characterize the intricacies of each target language phonology influenced by speakers' own nativity. 
% % Our method enriches this paradigm by 
% The proposed multilingual framework is enhanced with L1-aware speech representation, encapsulating the influence of speaker's own nativity.  

% phonological patterns to enhance the robustness and accuracy of mispronunciation detection in multiple languages.
% % along with lack of L2-data for the target language.
% The paper proposes a novel multilingual MDD architecture that 
